Fine-grained Appearance Transfer with Diffusion Models

Image-to-image translation (I2I), and particularly its subfield of appearance transfer, which seeks to alter the visual appearance between images while maintaining structural coherence, presents formidable challenges. Despite significant advancements brought by diffusion models, achieving fine-grained transfer remains complex, particularly in terms of retaining detailed structural elements and ensuring information fidelity. This paper proposes an innovative framework designed to surmount these challenges by integrating various aspects of semantic matching, appearance transfer, and latent deviation. A pivotal aspect of our approach is the strategic use of the predicted $x_0$ space by diffusion models within the latent space of diffusion processes. This is identified as a crucial element for the precise and natural transfer of fine-grained details. Our framework exploits this space to accomplish semantic alignment between source and target images, facilitating mask-wise appearance transfer for improved feature acquisition. A significant advancement of our method is the seamless integration of these features into the latent space, enabling more nuanced latent deviations without necessitating extensive model retraining or fine-tuning. The effectiveness of our approach is demonstrated through extensive experiments, which showcase its ability to adeptly handle fine-grained appearance transfers across a wide range of categories and domains. We provide our code at https://github.com/babahui/Fine-grained-Appearance-Transfer

==> preamble.tex <==
%
% --- inline annotations
%
% \usepackage[dvipsnames]{xcolor}
% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}


% %  teaser
% \let\oldtwocolumn\twocolumn
% \renewcommand\twocolumn[1][]{%
%     \oldtwocolumn[{#1}{
    
% \begin{center}
% \vspace{-1.5em}
% \includegraphics[width=0.98\textwidth]{images/teaser-11-18.pdf}
%     \captionof{figure}{The results of fine-grained appearance transfer using our method. The leftmost column displays the source images. On the right, the output images achieved by detailed appearance transfer corresponding to the target images (outlined in black), while preserving structural integrity. The examples at the bottom demonstrate our method's capability to transfer across various domains and categories.
%     % Exemplary results of fine-grained appearance transfer using our method. The left column displays the source images. Their visual appearances are transferred to the target images (outlined in black), achieving detailed appearance transfer while preserving structural elements. The examples at the bottom demonstrate the transfer across various domains and categories.
%     %Exemplary appearance transfer result with our method. The left column shows the source images, their appearances are transferred by leveraging target images (outlined in black) to achieve a detailed appearance transfer while preserving structural elements. The examples in the bottom demonstrate the transfer across various domains and categories.
%     }
%     \label{fig:teaser}
% \end{center}
%     }]
% }
